MuonTrap: Preventing Cross-Domain Spectre-Like Attacks by Capturing Speculative State

The disclosure of the Spectre speculative-execution attacks in January 2018 has left a severe vulnerability that systems are still struggling with how to patch. The solutions that currently exist tend to have incomplete coverage, perform badly, or have highly undesirable edge cases that cause application domains to break. MuonTrap allows processors to continue to speculate, avoiding significant reductions in performance, without impacting security. We instead prevent the propagation of any state based on speculative execution, by placing the results of speculative cache accesses into a small, fast L0 filter cache, that is non-inclusive, non-exclusive with the rest of the cache hierarchy. This isolates all parts of the system that can't be quickly cleared on any change in threat domain. MuonTrap uses these speculative filter caches, which are cleared on context and protection-domain switches, along with a series of extensions to the cache coherence protocol and prefetcher. This renders systems immune to cross-domain information leakage via Spectre and a host of similar attacks based on speculative execution, with low performance impact and few changes to the CPU design.

==> sections/attacks.tex <==
\section{Attack Examples}

\begin{attack}[Basic Prime and Probe]
\includegraphics[width=.95\linewidth]{figs/contextswitch}
\myparagraph{Requirements} Shared \ucache\ between victim and attacker processes 
\myparagraph{Vector} Priming the \ucache\ \textbf{(1)}, followed by loading of secret data \textbf{(2)}, and using that to evict data from the \ucache\ \textbf{(3)}
\myparagraph{Defense} Flush \ucache\ on context switches
\end{attack}

\noindent A \ucache\ protects against many attacks on the memory system other than the simple prime and probe of cache data used in the original Spectre proof of concept~\cite{Kocher2018spectre}. Here, we give examples of several of these attacks, the mechanisms by which they work, and how our speculative \ucache\ protects against them. This is not intended to be exhaustive. Instead, it is designed to illustrate key examples of the breadth of attacks one must protect against with a Spectre mitigation, allowing a reader to come up with similar attacks to cover the full scope.

\subsection{Basic Prime and Probe}

\noindent In a basic prime and probe attack using Spectre (\cref{attack:Basic Prime and Probe}), the attacker first primes the cache (in this case, the \ucache).
They then context switch to the victim and can work out some secret information if the attacker's data is evicted by the Spectre attack.
However, our design prevents this by flushing on context switches, which guarantees the attacker's data will never be in the \ucache, regardless of what the victim is forced to read.
Likewise, even in the presence of shared data, flushing the \ucache\ between the victim's execution and the context switch back to the attacker ensures that this data will no longer be in the cache, meaning neither presence nor absence can be used for the attacker's side channel.

\subsection{Inclusion Policy}
\noindent Making the \ucache{} inclusive or exclusive with respect to other levels of the cache hierarchy opens up a side channel whereby an attacker could force data to be in other caches through a speculative load, thereby evicting other data (inclusion) or force it to be evicted from other caches via a speculative load (exclusion), shown in \cref{attack:Inclusion Policy}.
\begin{attack}[Inclusion Policy]
\includegraphics[width=.95\linewidth]{figs/inclusivity}
\myparagraph{Requirements} Inclusion or exclusion with shared data between attacker and victim
\myparagraph{Vector} Priming the L1 cache \textbf{(1)}, followed by loading of secret data \textbf{(2)}, and using that to evict data indirectly from the L1 by using inclusion \textbf{(3)} or exclusion with shared data
\myparagraph{Defense} Non-exclusive, non-inclusive \ucache
\end{attack}


The act of bringing data into a \ucache{} should not affect state within other caches, so we guarantee neither exclusivity nor inclusivity with the \ucache\ with respect to other cache levels.
This means that when a \ucache{} miss occurs, data is fetched from the nearest location as usual and if that is another cache, it is left there too.

 
 \subsection{Coherence Attacks}

 
 \noindent Speculative data accesses can affect caches other than the \ucache\ even if we do not evict any data in higher cache levels when bringing data into the \ucache. This is because of the cache coherence protocol, which gives rise to another side channel (\cref{attack:Shared Data}).
  
 
 \begin{attack}[Shared Data]
 \includegraphics[width=\linewidth]{figs/coherencydiags2/no.pdf}
 
 \myparagraph{Requirements} Shared data between the attacker and victim, with write access for the attacker, or ability for the victim to perform speculative prefetching in the exclusive state or issue speculative write coherency requests~\cite{SpectrePrime}
 
 \myparagraph{Vector} Priming the cache \textbf{(1)} with a load, followed by tricking the victim into loading a secret \textbf{(2)} and using that to trigger a load \textbf{(3)} or store attempt to the same data~\cite{SpectrePrime}, increasing the time taken for the attacker to perform a store \textbf{(4)}
 
 \myparagraph{Defense} Reduced coherency speculation
 
 \end{attack}
 
If, in another core's cache, data which was in the exclusive state is now in shared, we can infer this by writing to it.
 Similarly, if data was in shared state but is now invalid~\cite{SpectrePrime}, we can detect this by reading it.
 This side-channel is more difficult to exploit than a standard Spectre attack because it isn't based on data eviction: shared data is required for the attacker and victim.
 However, we can leak information using shared read-only access by tricking the victim process into executing a speculative prefetch-exclusive, or even a write in some microarchitectures~\cite{SpectrePrime}, that preempts the architectural write with a coherency request, to invalidate data in the cache used by our attacker thread.
 
 We can address this by preventing changes in other cores' cache state during speculation.
 If a memory operation performed by speculative execution would result in a coherency state change in another core's cache, the instruction must wait until it is non-speculative (in our implementation, until all previous instructions have committed) or it gets squashed.
 To implement this we issue the memory operation speculatively and make it fail if it causes another cache to change coherency state, then repeat it non-speculatively if required.
 
 Still, this solution creates its own side-channel vulnerability if the attacker process is also executing speculatively: we can work out whether an address is in the victim's \ucache\ by issuing a speculative load (\cref{attack:\Ucache{} Coherency}).
 If the attacker's load takes longer than expected, we can infer that the data is in another \ucache\ in the exclusive state.
 Again, we need shared read access to data, but provided this is available then this is a side channel as easy to exploit as the cache coherency vulnerability itself.
 
 \begin{attack}[\Ucache{} Coherency]
 \includegraphics[width=\linewidth]{figs/coherencydiags2/delayatt.pdf}
 \myparagraph{Requirements} \Ucache\ with reduced coherency speculation, and shared data between the attacker and victim
 
 \myparagraph{Vector} Speculative load access by the victim to secret data \textbf{(1)} used to trigger an access to shared data \textbf{(2)}. This is followed by a load to an address the attacker knows will miss \textbf{(3)} causing a load to the same address accessed by the victim to be executed speculatively \textbf{(4)}, and thus be delayed \textbf{(5)}
 
 \myparagraph{Defense} Loading into the \ucache\ as shared, with asynchronous upgrade at commit (for performance).
 \end{attack}
 
 
 The fix for this involves preventing any speculative memory access from bringing in data in a non-shared state. This means that any \ucache\ is isolated from any other \ucache's behavior, and we need not check \ucache s on speculative load operations. We can still gain the benefits of a more complex MESI protocol by asynchronously upgrading loads on retirement to the E state, without introducing speculative side channels, as discussed in \cref{ssec:coherency}.
 
\subsection{TLB System}
 
\noindent  The TLB stores separate translations for each process, so there will be no shared data between different processes, and thus the presence of data within a TLB is not a valid side channel, unlike with an instruction or data cache. 
However, if the act of using secret data to trigger a TLB miss by the victim can evict the attacker's entries, by leaking different bits by evicting different TLB entries (see \cref{attack:TLB}).
 
 \begin{attack}[TLB]
 \includegraphics[width=.95\linewidth]{figs/tlb}
 \myparagraph{Requirements} Non-fully-associative TLB used for both attacker and victim processes
 \myparagraph{Vector} Priming the TLB \textbf{(1)}, followed by loading secret data into the \ucache\ \textbf{(2)}, and using that to perform a load that causes a TLB fill \textbf{(3)}
 \myparagraph{Defense} Speculative micro-TLB
 \end{attack}
 
This attack is still technically feasible even with a fully-associative TLB. This is because the victim could be made to conditionally load either an address with a TLB entry already present, or not present, based on the secret data. However, this would require the attacker to trick the victim into priming its own TLB, and for the attacker to have a complex Spectre gadget to be able to choose either a missing or non-missing TLB entry. This likely makes such an attack infeasible in practice unless the TLB is set associative.
 
 Regardless of whether this is possible, the TLB will be a very slow side-channel when compared with the data cache. Still, a speculative micro-TLB, as described in \cref{ssec:utlb}, can fully mitigate any possible attack.
 
 \subsection{Instruction Cache}
 
\noindent The data path is not the only way that speculative execution can leak secret data. We can instead use the instruction cache as the side channel, by using the data to branch to different addresses based on the secret's values (\cref{attack:Instruction Cache}).

 \begin{attack}[Instruction Cache]
 \includegraphics[width=.95\linewidth]{figs/icache}
 \myparagraph{Requirements} Non-fully-associative instruction cache, used by both attacker and victim processes
 \myparagraph{Vector} Priming the instruction cache \textbf{(1)} by the attacker, followed by loading of secret data \textbf{(2)} and using it to index into the instruction cache using an indirect branch \textbf{(3)}
 \myparagraph{Defense} \Ucache\ for instruction access
 \end{attack}

This attack is more complicated than using a data side channel, as the attacker's instructions used to time the execution of the evicted instruction may themselves alias with the target, and the attacker must time and execute valid instructions to test the cache's access time.
 It is, nevertheless, possible to infer data based upon it.
 


 
 
 %use the private data to load an instruction, then time execution of instructions which alias. This is more complicated as all instructions may alias, but may be possible, and can be also fixed using a speculative \ucache\ - keep the committed bit to write back, but coherency now simpler.
 
 \subsection{Prefetcher}

 
 
 \noindent Although prefetching~\cite{IntelPrefetchers,prefetcherbook,StridePrefetcher,Gruss:2016:PSA:2976749.2978356} is a form of speculation, it is not based on speculative execution, and therefore isn't directly subject to the same injection vulnerabilities that cause Spectre and Meltdown.
 However, prefetchers expose a side channel when they fetch data based on a speculative load.
 If an attacker loads a line into the \ucache\ speculatively, then the following line of data is prefetched into the L1 or L2, the attacker can infer information in the same way as with Spectre (\cref{attack:Prefetcher}). Prefetchers are important for performance, so we cannot disable them entirely.
 We instead remove this side channel by notifying prefetchers on commit, rather than speculative load, so the prefetcher sees the pattern it would have under in-order execution, as described in \cref{ssec:prefetcher}.

 \begin{attack}[Prefetcher]
 \includegraphics[width=\linewidth]{figs/prefetcher}
 \myparagraph{Requirements} Prefetcher with access to speculative instruction stream
 \myparagraph{Vector} Priming a cache featuring a prefetcher \textbf{(1)} by the attacker, followed by loading secret data \textbf{(2)} by the victim, who then loads an address to trigger the prefetcher to bring the next line into a non-speculative cache \textbf{(3)}
 \myparagraph{Defense} Prefetch on commit
 \end{attack}





\subsection{Multithreading}
 
 \begin{attack}[Multithreading]
 \includegraphics[width=\linewidth]{figs/smt}
 \myparagraph{Requirements} Concurrent access of the same \ucache\ by an attacker and victim process, with either a non-fully-associative \ucache\ or with data that both processes can read from the cache
 \myparagraph{Vector} Priming of the \ucache\ by an attacker \textbf{(1)} running concurrently with the victim, who performs a standard Spectre attack \textbf{(2,3)}
 \myparagraph{Defense} \Ucache\ per thread
 \vspace{-5pt}
 \end{attack}

\noindent  Provided we want to be able to run multiple threads on the same core from different processes simultaneously, each thread must have its own separate \ucache\ or partition of the \ucache, to prevent a further attack (\cref{attack:Multithreading}).

\subsection{Summary}

\noindent Here we have presented a subset of example attacks that could be used to extract information using speculative execution, and how the speculative \ucache\ can be used to prevent them. This is not intended to be exhaustive---it is instead to show the variety of different mechanisms that are available. We now move on to show performance impact of these protections on applications under simulation.

==> sections/microcache.tex <==

\section{Speculative \UCACHE}


%\myparagraph{Attack requirements} non-fully-associative caches or shared data, out-of-order execution
%\myparagraph{Attack vector} Eviction of data primed by an attacker process, as a result of speculative execution in a victim process, thus leaking secret data in the address of a cache access, or loading of shared data into the cache based on speculative execution on secret data in the victim process.
%\myparagraph{Defence} \Ucache

\noindent We prevent speculative execution from leaving a trace that can be used for side-channel attacks by adding a small, 1-cycle access L0 cache between the core and the L1 cache, which is cleared on context switches.
We force all speculative memory state to reside in the L0, meaning that other caches in the memory hierarchy contain only data that is non-speculative (i.e., it has been accessed by committed instructions only).
We call the L0 cache a \emph{speculative \ucache} and collectively refer to other caches in the hierarchy as \emph{non-speculative caches}.

With this new addition, speculative memory accesses propagate through the conventional cache system, but do not evict data from non-speculative caches and do not store any data within them.
Data may be copied back to the L1 cache when a load or store using a given cache line commits.
Although speculative data may be evicted before this point, it must not be written into any non-speculative cache.

Adding this small cache increases lookup time in the L1 cache by one cycle, due to the need to consult the \ucache{} before the L1.
However, its size means it can be faster than a conventional L1 cache in an out-of-order superscalar system, so for memory accesses with high temporal or spatial locality, we should expect that this system will slightly improve performance via hits to the \ucache, as well as give the security properties we require. 

In this section we first discuss the requirements and parameter space of the basic \ucache, before moving on to consider similar attacks on the memory system that don't directly use cache-line timing from the data cache, and how we can expand our strategy to further prevent such attacks.
Where we make design decisions to prevent a side-channel attack, we diagrammatically show the attack and introduce its requirements and vector, before describing how we use our strategy to prevent the given attack.


The overall architecture of our scheme, including extended defences against other Spectre-like attacks on the memory system, is given in \cref{fig:architecture}.

%Small caches have been looked at before for performance, but this is minor. Here, we wish to use them to achieve security correctness, while still allowing performance increases where possible.

\subsection{Behavior}

\noindent We use the \ucache{} to isolate speculative data from the existing cache hierachy, while still providing access to this data to improve performance. This means that higher levels of cache are not filled upon a miss (speculative or otherwise); instead this data is brought directly into the L0 \ucache. 

We only allow data to propagate into non-speculative caches if an instruction using that data has reached commit in the out-of-order processor pipeline: that is, if the data would have been loaded in the absence of speculative execution. We do this by adding a \emph{committed} bit to each \ucache{} line that is reset to zero when a cache line is brought in by a speculative instruction, or set to one when a cache line is brought in through a non-speculative instruction.
When loads and stores commit, the cache is accessed and the \emph{committed} bit for the cache line is set if it is zero, writing the data to the L1 in the process (for both operations).

The \ucache\ uses a write-through policy.
Although we could use a write-back policy, it complicates the cache flushing that is necessary on context switches (see \cref{sec:ucache:switch}).
By writing through, we know that all data in the \ucache\ can safely be thrown away at any point during execution.

\subsection{Parameters}

\noindent A \ucache\ can vary in terms of size and associativity. This has both performance and, in some cases, security implications.
We discuss these here before evaluating them in detail in \cref{sec:eval}.
We mandate that the \ucache{} is neither inclusive nor exclusive with respect to the rest of the cache system, to avoid opening a new side-channel.
To increase performance we require the \ucache\ to be virtually indexed.

\subsubsection{Cache Size}

% Tim: potential new start to this section.
The \ucache{} is the fastest cache in the system, with the ability to store both speculative and non-speculative data.
In terms of performance, we therefore want to size it as large as possible within the constraints of a 1-cycle access latency.

The \ucache\  should at least be large enough to support storing data for all current speculative execution: otherwise, data will be evicted from the cache before it is committed, and won't reach the L1 cache, limiting the amount of temporal locality we can exploit. Alternatively, the system could stall waiting for \ucache\ space, depending on replacement policy, but this would result in more state maintenance in the \ucache, as incorrectly speculated data would have to be evicted. This might lead us to believe that a \ucache\ should have at least as many cache lines as there are elements in a core's load queue. Ignoring aliasing from a possible set-associative indexing policy, and any evictions, this would guarantee that every element in the load queue will also be in the \ucache. 

Still, there is a trade-off between power and area, and performance here. A smaller, less associative cache will use less energy for lookup, and as the \ucache\ will be frequently accessed this is likely to be an important design constraint. This means that the smallest \ucache\ that doesn't lower performance may still be a useful design point, even if performance can be increased with larger \ucache{}s.
We evaluate the performance impact of different \ucache{} sizes in \cref{sec:eval:size}.

%However, there are two other factors at play here. The first is that there may be temporal locality, or spatial locality within cache lines, with accesses in the load queue, meaning fewer cache lines than load queue entries will be required for maximal performance. On the flip side, the \ucache\ gives the fastest access time in the system, and therefore it is beneficial to keep as much data in it as possible. This means that performance should increase even with more cache lines in the \ucache\ than the processor can speculatively access concurrently.


\subsubsection{Associativity}
\label{sec:ucache:assoc}
A set-associative or direct-mapped \ucache{} contains a side channel on a miss due to the use of address bits to choose a victim line for replacement.
An attacker could prime the \ucache{} with certain data, then infer information about the address of that data by causing it to be evicted.
\begin{attack}[Associativity]
\includegraphics[width=\linewidth]{figs/contextswitch}
\myparagraph{Requirements} Non-fully-associative \ucache
\myparagraph{Vector} Leaking of data from the \ucache\ itself, by priming \textbf{(1)} the \ucache\, followed by a load of secret data \textbf{(2)} and the use of it to load an address based on the data \textbf{(3)} to evict the primed data
\myparagraph{Defense} Clear the \ucache\ on a context switch
\end{attack}
A fully associative \ucache{} prevents conflict misses evicting speculative data, and therefore eliminates this side-channel because no address bits are used to determine the victim line.
However, a fully associative \ucache{} may not be desirable due to power, access time and capacity trade-offs.
Therefore, to implement a secure non-fully-associative \ucache, we must clear it on a context switch to prevent against Spectre-like attacks from other processes.
%If we are also directly using the \ucache\ to protect against within-process attacks such as Meltdown (not assumed by this scheme), we also need to entirely empty the \ucache\ on any mis-speculation, including of correctly loaded values, otherwise the eviction of correct data by incorrect data is itself a side channel.


\subsubsection{Inclusion Policy}
Making the \ucache{} inclusive or exclusive with respect to other levels of the cache hierarchy opens up a side channel whereby an attacker could force data to be in other caches through a speculative load, thereby evicting other data (inclusion) or force it to be evicted from other caches via a speculative load (exclusion).
\begin{attack}[Inclusion Policy]
\includegraphics[width=.95\linewidth]{figs/inclusivity}
\myparagraph{Requirements} Inclusion or exclusion with shared data between attacker and victim
\myparagraph{Vector} Priming the L1 cache \textbf{(1)}, followed by loading of secret data \textbf{(2)}, and using that to evict data indirectly from the L1 by using inclusion \textbf{(3)} or exclusion with shared data
\myparagraph{Defense} Non-exclusive, non-inclusive \ucache
\end{attack}
The act of bringing data into a \ucache{} should not affect state within other caches, so we guarantee neither exclusivity nor inclusivity with the \ucache\ with respect to other cache levels.
This means that when a \ucache{} miss occurs, data is fetched from the nearest location as usual and if that is another cache, it is left there too.

Higher levels of the cache hierarchy can be inclusive or exclusive with respect to each other.
However, these properties make write-through from the \ucache{} more complex.
When the L1 and L2 are exclusive, for example, we would have to send an invalidate signal to the L2 upon writing data to the L1.
When they are inclusive, we would have to make our writes and load commits write through to the inclusive L2.
Therefore, we guarantee neither in our implementation.

Here we assume that cache line sizes are the same at all levels of the cache hierarchy, so data from the \ucache\ can be used to fill any other cache.
If cache line sizes differ, the \ucache\ must take the size of the largest cache line in the system, and write through to this cache upon eviction of data.


\subsubsection{Addressing}
\label{sec:ucache:addr2}
The \ucache\ is accessible in a single cycle, so it is desirable to avoid virtual-address translation on access, which also avoids adding a new port to the TLB.
Clearing it on a context switch avoids aliasing between different physical addresses for shared virtual addresses across multiple processes.
However, the \ucache{} must be checked by the cache coherence logic, so it must be possible to index it by physical address.
We therefore tag each entry with both the virtual and physical address of the data and index the cache by the shared least significant bits of both.
This means it is virtually indexed from the CPU side and physically indexed from the memory side, to avoid translation.
We prevent virtual-address aliasing within a process by physically addressing upon a memory fill, which may overwrite an entry with a different virtual address but ensures that only one copy of each physical address exists at a time in the \ucache.



\subsection{\Ucache\ Protection Behavior}

\noindent In addition to the specific parameters of the \ucache, there are a number of properties we must ensure it obeys if speculative data is to be isolated from an attacker. These force us to prevent data from being written to any non-speculative cache unless it is committed by a thread, to clear the \ucache\ on a context switch, and to isolate threads running concurrently on the same core from each other. As a result of these protections, the \ucache\ must be part of any coherency mechanism of the system.


\subsubsection{Replacement}
On a miss in the \ucache{} we allow any cache line to be evicted, regardless of whether it has been committed.
Because stores write through to the L1, there is no dirty data in the \ucache, and therefore the choice of victim has only performance implications.
Our policy means that we do not distinguish between data that has not yet committed and data that was brought in by an earlier mis-prediction, allowing mis-speculated data to remain in the \ucache{} in case it is accessed in the near future.
However, this opens a vulnerability, albeit one that requires significant control over the victim.
\begin{attack}[Early Replacement]
\includegraphics[width=.95\linewidth]{figs/tobecommitted}
\myparagraph{Requirements} Some control of a victim thread for both correct and speculative execution, non-fully-associative \ucache
\myparagraph{Vector} Priming the \ucache\ \textbf{(1)}, followed by speculative but correct execution of a load by the victim that conflicts with the primed data \textbf{(2)}, followed by a conventional Spectre attack \textbf{(3,4)} before \textbf{(2)} commits, incorrectly leaving \textbf{(1)} in the L1 cache
\myparagraph{Defense} Software, fully associative \ucache, or blocking on eviction of uncommitted data
\end{attack}
This attack only applies to non-fully-associative \ucache{}s, requires complex control over both correct and speculative execution of the victim thread, extremely complex timing capabilities, and the ability to load as many secret values in a single speculative execution as the associativity of the \ucache. We therefore consider it no further here.
However, it is possible to remove this side channel by disallowing eviction of uncommitted data from the \ucache, or by forcing a reload of evicted data upon instruction commit.


\subsubsection{Context Switches}
\label{sec:ucache:switch}
\Cref{sec:ucache:assoc} described the importance of invalidating a set-associative or direct-mapped \ucache{} on a context switch and \cref{sec:ucache:addr} laid out the benefits of this approach in avoiding address translation on access.
Another benefit is that it gives a security feature unavailable even from a fully associative \ucache.
While Spectre uses data eviction as a side channel, which is unavailable from a fully associative cache, the existence of data in a cache can also be used as a side channel, provided we have shared data between the attacker and victim.
To prevent this, we must clear the cache to mask the vulnerability.
\begin{attack}[Shared Data]
\includegraphics[width=\linewidth]{figs/uncommittedshared}
\myparagraph{Requirements} Shared data
\myparagraph{Vector} Causing the victim to load secret data \textbf{(1)}, which it uses to load data shared with the attacker \textbf{(2)}, which the attacker then times an access to \textbf{(3)}
\myparagraph{Defense} Clear the \ucache\ on a context switch
\end{attack}
We implement cache invalidation efficiently by storing a \emph{valid} bit per cache line, in flip flops separate from the SRAM cache.
On a context switch, rather than having to access every SRAM block, which may take as many cycles as there are cache lines, we can invalidate the entire cache by clearing every \emph{valid} bit, which can be performed in parallel within a single cycle.
On lookup, any cache line with the \emph{valid} bit not set is ignored in the \ucache.
This is unconventional for caches, which normally store validity implicitly using coherency state in SRAM, but is necessary for fast invalidation of the cache, and the extra state is feasible considering the small size of a \ucache.
It is this fast invalidate that requires the \ucache{} to be write-through.

\newpage

\subsubsection{Multithreading Support}

Protection of the \ucache{} relies on isolating speculative data within the \ucache{} from threads from other processes.
This necessitates that when multiple processes are run concurrently via simultaneous multithreading on the same core, they must not be able to infer \ucache\ state about the other, otherwise information may leak between the two.
\begin{attack}[Multithreading]
\includegraphics[width=\linewidth]{figs/smt}
\myparagraph{Requirements} Concurrent access of the same \ucache\ by an attacker and victim process, with either a non-fully-associative \ucache\ or with data that both processes can read from the cache
\myparagraph{Vector} Priming of the \ucache\ by an attacker \textbf{(1)} running concurrently with the victim, who performs a standard Spectre attack \textbf{(2,3)}
\myparagraph{Defense} \Ucache\ per thread, or fully associative \ucache\ with isolation of shared data
\end{attack}
Defense for this attack once more points to a fully associative cache.
Alternatively, each thread must have its own separate \ucache\ or partition of the \ucache.
Still, in the presence of shared data, even with a fully associative \ucache, it may still be possible to leak information from one process to the other by the existence of data in the \ucache.
To prevent this, we need to avoid the attacker process from inferring existence of speculatively loaded data in the \ucache.
Indexing by virtual address and process ID would prevent data sharing directly between two processes. However, since we only allow one copy of each physical address in a \ucache\ at a time, access by one thread would cause eviction for the other, creating a side channel. It is therefore necessary in these cases to use separate \ucache s per thread.

\subsubsection{Cache Coherency}

The \ucache\ stores data that may not be in any other cache level, and therefore must be checked by any mechanisms to preserve coherence.
Without this, the \ucache\ could change program correctness by speculatively accessing data, whether the speculation is correct or not.
We explore attacks related to the coherence protocol in \cref{sssec:coherenceprevention}.

\subsection{Summary}

\noindent To prevent speculative data from being leaked within the memory system, we have added an extra layer of indirection into the cache hierarchy.
This \ucache{} sits between the core and the L1 data cache to store speculative data and is cleared on context switches.
We have described attacks relating directly to the \ucache{} and their defenses; the following section considers prevention of a host of similar attacks on other parts of the memory system using a similar strategy.



\section{Protection From Other Attacks}
\label{sec:otherattacks}

\noindent Protection against Spectre-like attacks will fail if other side channels can leak information.
In fact, in some cases a \ucache\ on its own can make attacks easier.
We therefore consider how to mitigate against these attacks, either by augmenting \ucache s to further prevent information leakage, or through modifications elsewhere in the memory system.


\subsection{Coherence Attack Prevention}
\label{sssec:coherenceprevention}

\noindent Speculative data accesses can affect caches other than the \ucache\ even if we do not evict any data in higher cache levels when bringing data into the \ucache. This is because of the cache coherence protocol, which
gives rise to another side channel attack.




\begin{attack}[Shared Data]
\includegraphics[width=\linewidth]{figs/coherencydiags2/no.pdf}

\myparagraph{Requirements} Shared data between the attacker and victim, with write access for the attacker, or ability for the victim to perform speculative prefetching in the exclusive state or issue speculative write coherency requests~\cite{SpectrePrime}

\myparagraph{Vector} Priming the cache \textbf{(1)} with a load, followed by tricking the victim into loading a secret \textbf{(2)} and using that to trigger a load \textbf{(3)} or store attempt to the same data~\cite{SpectrePrime}, increasing the time taken for the attacker to perform a store \textbf{(4)}

\myparagraph{Defense} Reduced coherency speculation

\end{attack}
If, in another core's cache, data which was in the exclusive state is now in shared, we can infer this by writing to it.
Similarly, if data was in shared state but is now invalid~\cite{SpectrePrime}, we can detect this by reading it.
This side-channel is more difficult to exploit than a standard Spectre attack because it isn't based on data eviction: shared data is required for the attacker and victim.
However, we can leak information with only shared read-only access by tricking the victim process into executing a speculative prefetch-exclusive, or even a write in some microarchitectures~\cite{SpectrePrime}, that preempts the architectural write with a coherency request, to invalidate data in the cache used by our attacker thread.

We can address this attack either by preventing changes in other cores' cache state during speculation (i.e., when executing a speculative load), or by rolling back any changes after a failure of speculation.
We choose the former approach for simplicity.
If a memory operation performed by speculative execution would result in a coherency state change in another core's cache, the instruction must wait until it is non-speculative (i.e., all previous instructions have committed) or it gets squashed.
To implement this we issue the memory operation speculatively and make it fail if it causes another cache to change coherency state, then repeat it non-speculatively if required.


%Three problems: don't want to change exclusive/modified data in another cache to be shared, as we can then time this by performing a write. Similarly, don't want to move from shared to invalidate by a prefetch exclusive in the attack thread. Latter we can solve by making prefetch exclusives non-speculative. We can solve both by either rolling back any coherency changes, but this requires complex state management and complicates protocol, or by making memory operations non-speculative if they cause any changes in state. We do the latter. 

Still, this solution creates its own side-channel vulnerability if the attacker process is also executing speculatively: we can work out whether an address is in the victim's \ucache\ by issuing a speculative load.

\begin{attack}[\Ucache\ Coherency]
\includegraphics[width=\linewidth]{figs/coherencydiags2/delayatt.pdf}
\myparagraph{Requirements} \Ucache\ with reduced coherency speculation, and shared data between the attacker and victim

\myparagraph{Vector} Speculative load access by the victim to secret data \textbf{(1)} used to trigger an access to shared data \textbf{(2)}. This is followed by a load to an address the attacker knows will miss \textbf{(3)} causing a load to the same address accessed by the victim to be executed speculatively \textbf{(4)}, and thus be delayed \textbf{(5)}

\myparagraph{Defense} Uncommitted data clearing in the \ucache\ on mis-speculation
\end{attack}

If the attacker's load takes longer than expected, we can infer that the data is in another \ucache\ in the exclusive state.
Again, we need shared read access to data, but provided this is available then this is a side channel as easy to exploit as the cache coherency vulnerability itself. To avoid this, we must empty any uncommitted state in the \ucache\ following a mis-speculation in the attached processor. The penalty we pay here is that any data accessed via a mis-speculation that is then subsequently used in correct execution must be reloaded.

This prevents any non-transient~\cite{4318988} side channel from inferring coherence information. However, if the victim has not yet discovered that it is executing down a mis-speculated path (for example, execution is blocked on an earlier branch-determining cache miss), then the attacker's load will execute before the victim evicts its own \ucache. Still, to gain any timing information from this requires complex scheduling capabilities, unlike any of the other attacks presented in this paper. If the attacker loads the shared data before the victim, executes non-speculatively, or loads the shared data once the victim has restarted execution, the attack will be unsuccessful. This means that it is unclear whether the attack is practical, or even possible, and we therefore consider further mitigations to prevent this unnecessary.

%We therefore allow speculative execution to move exclusive data in another process's \ucache\ into the invalidated state, so that the attacker thread cannot infer existence of data in a \ucache. We could allow both to move into the shared state, which would hide the existence of the other core's data entirely provided the attacker cannot write to the data. However, if the attacker can write to it, a write following the read would be spuriously slow, due to requiring a coherency upgrade, thus giving a side channel. Thus, we must pretend that the data does not exist in the other \ucache\ and give exclusive access to any uncommitted data requested.

% This is still vulnerable to an attack where the attacker brings shared data into its cache, and then before it commits this load, brings the data speculatively into the victim's cache. Through a second access, the attacker can then infer that it is no longer in possession of an exclusive copy of the data. However, this requires the ability to control concurrent execution of both attacker and victim with very precise timing properties, and is therefore likely to be an unrealistic attack vector in practice. We can protect against this by checking the state of loaded data when it is committed in the \ucache. If it is in the invalidated state, we can proactively issue another request to it, which will bring the data in in the exclusive state provided it hasn't been committed in another \ucache. This means that a victim speculatively loading a value after an attacker speculatively loads it won't result in the attacker's data being in the invalid state after speculative execution ends.

%This might seem like it's open to a ping-pong attack, where the victim is forced to load the data, followed by the attacker, followed by the victim, upon which the attacker can issue a timing attack for its second load to infer it isn't in its own cache. But this relies on the second victim load occurring after the attacker's first load, and the second attacker load occurring before the first attacker load has committed. In all other cases, the non-speculative defence will fix the vulnerability. We believe that the only way this can be caused is by a deliberate cache stall from an instruction before the first attacker load, which will be the critical path in execution and thus mask out any timeable characteristics of the two loads. [TODO: this is complicated as.]

%To fix this, we allow a speculative thread to invalidate data read from a \ucache\ in the exclusive state provided it is uncommitted. Another approach would be to clear 

%Finally, we also have the issue that if one thread is made to speculatively access data, and gets it in the exclusive state, an attacker thread bringing in the same data will get it in the shared state, so any writes to it will be delayed. Only viable if the attacker has write access to the shared data, again. We can either clear data on misspeculation, assuming attacks can't be done in realtime, or we can allow any read access from one thread to invalidate data in another \ucache, provided it is uncommitted. We choose the latter approach to allow misspeculated data to be left in a \ucache.

%This approach relies on a coherency protocol not introducing side channels that imply existence of data within a \ucache. This means that the coherency protocol's execution must take the same amount of time regardless of data's existence in the \ucache\ in an uncommitted state. The cache system can still forward values from committed state, for example from another private L1, however. %This is almost certain to be true for a snoopy protocol without inclusion, but care must be taken with directory protocols to ensure this.

\subsection{TLB System}


\noindent Fully associative TLBs prevent side-channels from a TLB access between two processes in the same manner as a fully-associative cache (see \cref{sec:ucache:assoc}).
However, in set-associative and direct-mapped TLBs we need to prevent eviction of non-speculative entries with speculative translations.
Though Spectre~\cite{Kocher2018spectre} itself does not attack the TLB, the attack vector is comparable, though likely more difficult to exploit.

\newpage
\begin{attack}[TLB]
\includegraphics[width=.95\linewidth]{figs/tlb}
\myparagraph{Requirements} Non-fully-associative TLB, used for both attacker and victim processes
\myparagraph{Vector} Priming the TLB \textbf{(1)}, followed by loading secret data into the \ucache\ \textbf{(2)}, and using that to perform a load that causes a TLB fill \textbf{(3)}
\myparagraph{Defense} Fully associative TLB, or speculative micro-TLB
\end{attack}
We can avoid this attack by performing a page-table walk on a miss in the \ucache{} and TLB, then storing translation information with the cache line in the \ucache{}, since we already store the virtual and physical page tags.
We would then write the translation information back to the TLB on commit.

However, speculative accesses within the same page but for different cache lines would trigger two TLB accesses, and potentially two page-table walks, which we wish to avoid for performance reasons.
We could limit this behavior by either checking all \ucache\ entries for a page match on a miss in the TLB, or by storing speculative state in a small, fully associative micro-TLB, and preventing its escape by using a committed bit similar to that in the \ucache.
This latter solution results in hardware similar to that used for the micro-TLBs in many conventional Arm systems~\cite{microTLB}, with the addition of the committed bit.

Hardware page-table walks triggered from speculative instructions can write into caches.
We must also, therefore, prevent side channels occurring through this mechanism.
Although we can enforce that these memory accesses go through a \ucache, working out when a page-table-walker cache entry should be committed is complex, as there is no one-to-one correspondence between executed instructions and page-table entries.
We must, therefore, on commit retranslate any instructions that caused page-table misses: these entries are likely to be in the \ucache\ at this point, and can be written back to the L1 as a result of the non-speculative retranslation.

\subsection{Instruction Cache}

\noindent Though the instruction cache was not used as an attack vector for the original Spectre attack~\cite{Kocher2018spectre}, it is possible to leak speculative information in a similar manner to attacking the data cache.
An attacker can cause a victim process to jump to a memory location based on the value of secret data, and then infer this information by timing instruction access. 
\newpage
\begin{attack}[Instruction Cache]
\includegraphics[width=.95\linewidth]{figs/icache}
\myparagraph{Requirements} Non-fully-associative instruction cache, used by both attacker and victim processes
\myparagraph{Vector} Priming the instruction cache \textbf{(1)} by the attacker, followed by loading of secret data \textbf{(2)} and using it to index into the instruction cache using an indirect branch \textbf{(3)}
\myparagraph{Defense} \Ucache\ for instruction access
\end{attack}
This attack is more complicated than using a data side channel, as the attacker's instructions used to time the execution of the evicted instruction may themselves alias with the target, and the attacker must time and execute valid instructions to test the cache's access time.
It is, nevertheless, possible to infer data based upon it.

We can fix this side channel in the same way that we fix the data side channel: by using a speculative \ucache\ for instructions in addition to that for data.
This is comparatively simpler because there is no cache coherency for read-only data, and so we only need to set the committed bit on committing an instruction and throw away any data evicted without this bit set.
We therefore do not have to clear the instruction \ucache\ on a speculation failure, but only on a context switch.


%use the private data to load an instruction, then time execution of instructions which alias. This is more complicated as all instructions may alias, but may be possible, and can be also fixed using a speculative \ucache\ - keep the committed bit to write back, but coherency now simpler.

\subsection{Prefetcher}
\label{ssec:prefetcher}


\noindent Although prefetching~\cite{IntelPrefetchers,prefetcherbook,StridePrefetcher} is a form of speculation, it is not based on speculative execution, and therefore isn't directly subject to the same injection vulnerabilities that cause Spectre and Meltdown.
However, prefetchers expose a side channel when they fetch data based on a speculative load.
If an attacker loads a line into the \ucache\ speculatively, then the following line of data is prefetched into the L1 or L2, the attacker can infer information in the same way as with Spectre.
On the other hand, prefetchers are very important for performance, so we cannot disable them entirely.
\begin{attack}[Prefetcher]
\includegraphics[width=\linewidth]{figs/prefetcher}
\myparagraph{Requirements} Prefetcher with access to speculative instruction stream
\myparagraph{Vector} Priming a cache featuring a prefetcher \textbf{(1)} by the attacker, followed by loading secret data \textbf{(2)} by the victim, who then loads an address to trigger the prefetcher to bring the next line into a non-speculative cache \textbf{(3)}
\myparagraph{Defense} Prefetch on commit
\end{attack}
To combat this attack, we can notify any L1 prefetcher of a load when it actually commits (gets written into the L1).

However, this policy will not work for the L2 cache, as if we assume a write-back policy for the L1 cache, the observed stream of loads at the L2 will be significantly out-of-order, and much later than their true execution. 
We must therefore provide higher level caches with a notification channel to provide information on in-order memory accesses, thus providing stronger constraints even than typical setups without a \ucache. When a load is committed in the speculative \ucache, prefetchers at each level in the cache hierarchy can be notified. However, not every memory access would have accessed, for example, the L2, and so not every commit needs to be sent to the L2 prefetcher. To reduce the number of messages sent to the system's caches, we can tag memory accesses in the speculative \ucache\  with the cache level they came from. When a load is committed in the \ucache, we read off from this which cache it was originally accessed from, and notify the prefetcher at that level. We then reset the tag, to prevent duplicate notifications which otherwise would not reach the relevant cache level.

\subsection{Within-Process Attack Prevention}
\label{ssec:meltdownprevent}

\noindent Although we assume that permissions bits are checked on memory accesses before bringing them even into the \ucache, protecting against Meltdown-style attacks~\cite{Lipp2018meltdown}, we could instead use the \ucache{} to protect against within-process attacks.
\begin{attack}[Meltdown]
\includegraphics[width=\linewidth]{figs/meltdown}
\myparagraph{Requirements} Delayed permissions checks on speculative memory accesses
\myparagraph{Vector} Priming the \ucache\ \textbf{(1)} by the attacker, followed by the attacker themselves loading secret data \textbf{(2)} and using it to load an address based on the data \textbf{(3)} to evict the primed data
\myparagraph{Defense} \Ucache\ clearing on mis-speculation
\end{attack}
The solution to this attack is to invalidate the \ucache{} not only on a context switch, but also as a result of any misprediction, meaning the state change within the \ucache\ is no longer visible once we return to code which will commit.
Further, this clearing of the \ucache\ is a stronger condition than is necessary for coherence attack prevention in \cref{sssec:coherenceprevention}: while for the latter, we need only clear all uncommitted data from the \ucache, for the former, we must clear all data, to prevent eviction of other data itself being used as a side channel, from the \ucache\ on a mis-speculation.


\subsection{Summary}

\noindent A basic \ucache\ in front of the L1 data cache, while able to defend against traditional Spectre attacks, can still allow information leakage through the cache hierarchy. We must therefore impose further constraints on the cache coherence protocol, add \ucache s to the TLB system and instruction cache, and prevent data leakage via the prefetcher, for our system to be secure against other similar attacks. Further, if we wish to protect against Meltdown attacks, it is possible to do this provided a \ucache\ is emptied on mis-speculation.

The following sections evaluate the overheads of adding these features, along with \ucache\ overheads more generally.

